ProAlign: Progressive Positional and Prototype-Guided Alignment for Aerial-Ground Person Re-Identification

Aerial-Ground Person Re-Identification (AG-ReID) aims to match pedestrian images captured by unmanned aerial vehicles (UAVs) and ground-based surveillance cameras. The task remains highly challenging due to severe viewpoint discrepancies, frequent occlusions, and substantial domain gaps between aerial and ground imagery. Beyond these observable factors, existing methods often overlook two fundamental structural issues: cumulative positional drift during hierarchical feature extraction and semantic inconsistency across cross-view feature distributions. To address these challenges, we propose ProAlign, a Progressive Positional and Prototype-Guided Alignment Network for AG-ReID. ProAlign comprises two key components: a Layer-wise Progressive Positional Embedding (LPPE) module and a View-Aware Prototype Contrastive Learning (PCL) module. LPPE performs adaptive positional calibration throughout transformer layers by employing conditional positional encoding in shallow layers to mitigate local spatial distortions, while introducing learnable static positional embeddings in deeper layers to reinforce global semantic priors. Meanwhile, PCL maintains view-specific aerial and ground prototypes for each identity and enforces cross-view semantic consistency via a dual-prototype contrastive objective. Extensive experiments on CARGO and two real-world AG-ReID benchmarks demonstrate the effectiveness of ProAlign, achieving state-of-the-art overall retrieval performance on CARGO with improvements of 1.60% in Rank-1 accuracy and 5.01% in mAP over the strongest competing methods.

==> method.tex <==
\section{Methodology}
\subsection{Overview}
The overall framework of the \textbf{Progressive Positional and Prototype-Guided Alignment Network (ProAlign)}, illustrated in Fig.~\ref{fig:model}, is built upon a ViT-Base backbone and designed to address spatial degradation and semantic inconsistency under complex aerial-ground multi-view conditions. Inspired by the success of the View-Decoupled Transformer (VDT)~\cite{dosovitskiy2020image}, we adopt the VDT architecture as the foundation of ProAlign, which effectively captures both global semantics and fine-grained structural cues. Following its design, we introduce an additional view token to model viewpoint-specific information. The token sequence during training is defined as:
\begin{equation}
\left[ \mathbf{X}_{\text{cls}}, \mathbf{X}_{\text{view}}, \mathbf{X}_{\text{img}} \right] 
= \text{VDT}\left( \left[ \mathbf{X}_{\text{cls}}, \mathbf{X}_{\text{view}}, \text{tokenize}(\mathbf{X}_{\text{img}}) \right] \right),
\end{equation}
where $\mathbf{X}_{\text{cls}}$, $\mathbf{X}_{\text{view}}$, and $\mathbf{X}_{\text{img}}$ represent the class token, view token, and image tokens, respectively. 

To improve geometric robustness and prevent cumulative positional drift, we integrate a \textbf{Layer-wise Progressive Positional Embedding (LPPE)} module into the transformer layers. This module applies depth-adaptive positional calibrations—utilizing conditional encodings in shallow layers and static embeddings in deep layers—to mitigate pose-induced geometric distortions iteratively. In addition, we introduce a \textbf{View-Aware Prototype Contrastive Learning (PCL)} module during training, which explicitly models identity distributions across aerial and ground views. PCL maintains quality-weighted prototypes to dynamically pull samples toward consistent identity subspaces, allowing the model to bridge the systematic cross-view gap while suppressing background noise and occlusion artifacts. Overall, ProAlign integrates LPPE and PCL, jointly optimizing for classification accuracy, layer-wise spatial stability, and robustness to extreme view variations. This synergy enables ProAlign to show a strong re-identification ability in severe aerial-ground variations.

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{fig2.png}
   \caption{\textbf{Overview of the ProAlign architecture.} Given aerial or ground-view inputs, ProAlign first extracts patch tokens and processes them through transformer layers equipped with Layer-wise Progressive Positional Embedding (LPPE) for depth-adaptive spatial correction. In parallel, the View-Aware Prototype Contrastive Learning (PCL) module maintains separate aerial and ground prototypes, guiding cross-view identity alignment and suppressing low-quality features.}
   \label{fig:model}\vspace{-1em}
\end{figure}

\subsection{Layer-wise Progressive Positional Embedding}
To address the spatial misalignment problem in person re-identification, we design a Layer-wise Progressive Positional Embedding (LPPE) module that explicitly models geometric variations arising from viewpoint discrepancies. By dynamically injecting positional corrections at each layer, the module prevents initial spatial offsets from compounding and corrupting deep representations. As illustrated in Fig.\,\ref{fig:model}, the LPPE modules are integrated into each transformer block to build a hierarchical, depth-adaptive alignment capability. The LPPE modules at shallower layers focus on compensating for local spatial distortions, while those at deeper layers are responsible for reinforcing global semantic positional priors.

The core idea of the LPPE module is to apply distinct positional encoding strategies based on the depth of the transformer. In the early layers (the first half of the network), spatial offsets are highly localized and tied to texture patterns. Therefore, we employ Conditional Positional Encoding (CPE). The CPE dynamically generates positional embeddings conditioned on the local neighborhood of the input patches using a depthwise convolution. For a given patch feature map $\mathbf{F} \in \mathbb{R}^{C \times H \times W}$, the shallow positional embedding $\mathbf{P}_{\text{CPE}}$ is formulated as:
\begin{equation}
    \mathbf{P}_{\text{CPE}} = \text{DWConv}(\mathbf{F}),
\end{equation}
where $\text{DWConv}(\cdot)$ denotes a $3 \times 3$ depthwise convolution with zero-initialized weights and biases. This dynamic generation allows the network to adaptively compensate for local spatial misalignments specific to each input image.

In contrast, the deeper layers of the ViT encode highly abstract, globally entangled representations. To align these deep features, we transition to learnable Static Positional Embeddings. Instead of conditioning on local patches, we initialize a set of independent, layer-specific static embeddings $\mathbf{P}_{\text{Static}} \in \mathbb{R}^{1 \times N \times D}$, which act as a global semantic anchor to guide the high-level features toward a canonical spatial layout. 

To ensure that the injection of these positional corrections does not disrupt the rich representations inherited from pretrained weights, we introduce a learnable gating mechanism. The calibrated patch feature $\mathbf{F}_{\text{final}}^{(l)}$ for the $l$-th layer is obtained by a gated residual fusion:
\begin{equation}
    \mathbf{F}_{\text{final}}^{(l)} = \mathbf{F}^{(l)} + g_l \cdot \mathbf{P}^{(l)},
\end{equation}
where $\mathbf{P}^{(l)}$ is the positional embedding (either $\mathbf{P}_{\text{CPE}}$ or $\mathbf{P}_{\text{Static}}$) at layer $l$, and $g_l$ is a learnable scalar initialized to zero. This gating strategy ensures that LPPE progressively phases in its spatial corrections over the course of training, dynamically adapting to complex scenes with large cross-view deformations.

\subsection{View-Aware Prototype Contrastive Learning}
In aerial-ground person re-identification, the drastic viewpoint changes create a systematic distributional gap between aerial and ground representations of the same identity. Relying solely on sample-to-sample alignment often fails due to heavy occlusions and noise. To address this issue, we propose the \textbf{View-Aware Prototype Contrastive Learning (PCL)} module, which explicitly models population-level identity distributions to bridge the semantic gap across views. PCL maintains a momentum-updated memory bank that anchors each identity to a shared prototype space, dynamically suppressing irrelevant or noisy samples from polluting the global representation.

Specifically, during training, we construct a view-conditioned prototype memory bank. For each identity $c$, we maintain two distinct prototypes corresponding to the two viewpoints: an aerial prototype $\mathbf{p}_c^{\text{aerial}} \in \mathbb{R}^D$ and a ground prototype $\mathbf{p}_c^{\text{ground}} \in \mathbb{R}^D$. To prevent occluded or low-quality samples from degrading the prototypes, we introduce a quality-weighted momentum update mechanism. The quality weight $w_i$ for the $i$-th sample feature $\mathbf{f}_i$ belonging to class $c$ in view $v$ is determined by its similarity to the current prototype:
\begin{equation}
    w_i = \max\left(0, \mathbf{f}_i \cdot \mathbf{p}_c^v \right).
\end{equation}
By applying a ReLU-like clamp, samples with negative similarities—often corresponding to severe occlusions or heavy background interference—are assigned a weight of zero and discarded from the update process. 

The prototypes are then updated using a momentum strategy. Let $\overline{\mathbf{f}}_c^v$ be the quality-weighted mean of the valid samples for class $c$ and view $v$ within the current mini-batch. The prototype is updated as:
\begin{equation}
    \mathbf{p}_c^v \leftarrow \text{Norm} \left( (1 - m) \cdot \mathbf{p}_c^v + m \cdot \overline{\mathbf{f}}_c^v \right),
\end{equation}
where $m \in [0, 1)$ denotes the momentum coefficient, and $\text{Norm}$ represents $\ell_2$ normalization. This weighted strategy ensures the prototypes robustly represent the most discriminative and visible features of each identity.

During the forward pass, these high-quality prototypes act as anchors for contrastive learning. By drawing each sample closer to its corresponding prototypes in both the intra-view and cross-view spaces, the network is forced to learn viewpoint-invariant representations. It is important to emphasize that this prototype memory bank is utilized only during the training phase to structure the feature space globally, meaning it introduces no additional computational overhead during inference.

\subsection{Loss Function and Optimization}
Our model is trained using a composite loss function designed to optimize identity discrimination, layer-wise spatial stability, and cross-view feature-level alignment. In addition to the standard ID classification loss $\mathcal{L}_{\text{id}}$ and the Triplet loss $\mathcal{L}_{\text{tri}}$ commonly employed in ReID tasks, we introduce a smoothness regularization loss $\mathcal{L}_{\text{smooth}}$ and a prototype contrastive loss $\mathcal{L}_{\text{pcl}}$.

\textbf{Smoothness Regularization Loss.} To enhance the stability of the LPPE module's static embeddings in the deep layers, we introduce a regularization term as the smoothness loss $\mathcal{L}_{\text{smooth}}$. This loss discourages adjacent layers from learning drastically different positional biases, thereby promoting a progressive, geometrically plausible refinement of features. It is defined as the mean squared error between the static positional embeddings of consecutive deep layers:
\begin{equation}
    \label{eq:smooth}
    \mathcal{L}_{\text{smooth}} = \sum_{l \in \text{Static Layers}} \left\| \mathbf{P}_{\text{Static}}^{(l)} - \mathbf{P}_{\text{Static}}^{(l+1)} \right\|_2^2.
\end{equation}
By penalizing abrupt spatial shifts between layers, this constraint ensures that the global semantic alignment refines gradually, avoiding over-fitting to meaningless layer-wise oscillations.

\textbf{Prototype Contrastive Loss.} To enforce population-level semantic alignment across the aerial and ground domains, we formulate a dual-prototype InfoNCE loss, denoted as $\mathcal{L}_{\text{pcl}}$. This loss comprises two components: an intra-view alignment term $\mathcal{L}_{\text{intra}}$ and a cross-view alignment term $\mathcal{L}_{\text{cross}}$. Let $\mathbf{f}_i$ be a sample feature in view $v$, with class label $c$. The network is optimized to identify the positive prototype $\mathbf{p}_c$ against all other negative identity prototypes $\mathbf{p}_k$ maintained in the memory bank. The InfoNCE loss for a specific target view $t$ is computed as:
\begin{equation}
    \label{eq:infonce}
    \mathcal{L}_{\text{InfoNCE}}(\mathbf{f}_i, t) = -\log \frac{\exp(\mathbf{f}_i \cdot \mathbf{p}_c^t / \tau)}{\sum_{k=1}^{C} \exp(\mathbf{f}_i \cdot \mathbf{p}_k^t / \tau)},
\end{equation}
where $\tau$ is the temperature hyper-parameter, and $C$ is the total number of initialized classes in the bank. 

The intra-view loss $\mathcal{L}_{\text{intra}}$ anchors the sample to its native viewpoint prototype ($t=v$), ensuring local consistency. Crucially, the cross-view loss $\mathcal{L}_{\text{cross}}$ forces the sample to align with the prototype of the opposite viewpoint ($t=1-v$). The overall contrastive loss is the weighted sum of both constraints:
\begin{equation}
    \mathcal{L}_{\text{pcl}} = \frac{1}{N} \sum_{i=1}^{N} \Big( \mathcal{L}_{\text{InfoNCE}}(\mathbf{f}_i, v) + \gamma \mathcal{L}_{\text{InfoNCE}}(\mathbf{f}_i, 1-v) \Big),
\end{equation}
where $N$ is the batch size, and $\gamma$ regulates the cross-view alignment strength. This dual objective explicitly bridges the domain gap, forcing the model to discard view-specific noise and extract robust, identity-consistent cues.

\textbf{Overall Loss.} The ProAlign model is trained end-to-end by minimizing a comprehensive loss function that aggregates the aforementioned components:
\begin{equation}
    \mathcal{L}_{\text{total}} = \mathcal{L}_{\text{id}} + \mathcal{L}_{\text{tri}} + \alpha \mathcal{L}_{\text{smooth}} + \beta \mathcal{L}_{\text{pcl}},
\end{equation}
where $\alpha$ and $\beta$ are hyper-parameters used to adjust the weight of the smoothness regularization and the prototype contrastive learning, respectively. This joint optimization framework encourages the learning of highly discriminative representations that are intrinsically resilient to cumulative spatial drift and systematic cross-view discrepancies.
